Characteristic times for gap relaxation and heat escape in nanothin NbTi superconducting filaments: thickness dependence and effect of substrate

We measured the temporal voltage response of NbTi superconducting filaments with varied nanoscale thicknesses to step current pulses that induce non-equilibrium superconducting states governed by a hot-spot mechanism. Such detected voltage emerges after a delay time td, which is intimately connected to the gap relaxation and heat escape times. By employing time-dependent Ginzburg-Landau theory to link the delay time to the applied current, we determined that the gap relaxation time depends linearly on film thickness, aligning with the acoustic mismatch theory for phonon transmission at the superconductor-substrate interface. We thereby find a gap relaxation time of 104 ps per nm of thickness for NbTi films on polished sapphire. We further show that interfacial interaction with the substrate significantly impacts the gap relaxation time, with observed values of 9 ns on SiOx, 6.8 ns on fused silica, and 5.2 ns on sapphire for a 50 nm thick NbTi strip at T = 5.75 K. These insights are valuable for optimizing superconducting sensing technologies, particularly the single-photon detectors that operate in the transient regime of nanothin superconducting bridges and filaments

==> coverletter.tex <==
Dear Editor, 

We hereby submit our manuscript "Characteristic times for gap relaxation and heat escape in nanothin NbTi superconducting filaments: thickness dependence and effect of substrate" for publication in Nanomaterials. 

In this work, we detail the resistive state of superconducting nanofilaments under biasing current pulses, that induce non-equilibrium superconducting states governed by a hot-spot mechanism. We measure a delay time t$_{d}$ upon which the nonzero voltage sets in, which is intimately connected to the gap relaxation and heat escape times. Those timescales are critical for the operation of superconducting sensors and electronics, but have been scarcely directly measured to date.

After a systematic analysis for a range of currents, temperatures, film thicknesses and different substrates, we report that the gap relaxation and heat escape times depend linearly on film thickness, aligning with the acoustic mismatch theory for phonon transmission at the superconductor-substrate interface. We thereby find a gap relaxation time of 104 ps per nm of thickness for NbTi films on polished sapphire. We further show that interfacial interaction with the substrate significantly impacts the gap relaxation time, with observed values of 9 ns on SiO$_{x}$, 6.8 ns on fused silica, and 5.2 ns on sapphire for a 50 nm thick NbTi strip at $T = 5.75$~K. 

Since these measurements and insights are valuable for optimizing superconducting sensing technologies, particularly the single-photon detectors and bolometers that operate in the transient regime of nanothin superconducting bridges and filaments, we expect our paper to be of immediate interest to the readership of Nanomaterials. We remain at your disposal should you require any further information regarding this submission. 

Yours sincerely, 
Authors


%POSSIBLE REFEREES %%%%%%%%%%%%%%%%%

Rosa Cordoba, University of Valencia, Spain, rosa.cordoba@uv.es, expert in transport measurements on superconducting nanostructures. 

Dieter Koelle, University of Tuebingen, Germany, koelle@uni-tuebingen.de, expert in superconducting nanosensors.

Vladimir Fomin, IFW Dresden, Germany, v.fomin@ifw-dresden.de, expert in theoretical simulations of superconductivity.

Boldizsar Janko, University of Notre Dame, USA, bjanko@nd.edu, expert in theory of superconductivity

Andrea Perali, University of Camerino, Italy, andrea.perali@unicam.it, expert in theory of superconductivity

Yukio Hasegawa, University of Tokyo, Japan, hasegawa@issp.u-tokyo.ac.jp, expert in Scanning probe and transport measurements on nanoscale superconductors




